ChemToolAgent: The Impact of Tools on Language Agents for Chemistry Problem Solving

To enhance large language models (LLMs) for chemistry problem solving, several LLM-based agents augmented with tools have been proposed, such as ChemCrow and Coscientist. However, their evaluations are narrow in scope, leaving a large gap in understanding the benefits of tools across diverse chemistry tasks. To bridge this gap, we develop ChemToolAgent, an enhanced chemistry agent over ChemCrow, and conduct a comprehensive evaluation of its performance on both specialized chemistry tasks and general chemistry questions. Surprisingly, ChemToolAgent does not consistently outperform its base LLMs without tools. Our error analysis with a chemistry expert suggests that: For specialized chemistry tasks, such as synthesis prediction, we should augment agents with specialized tools; however, for general chemistry questions like those in exams, agents' ability to reason correctly with chemistry knowledge matters more, and tool augmentation does not always help.

==> cctask.tex <==
% \subsubsection{\cctask}
% \hs{remove this section/task for the following reasons? (1) why these 4 tasks is not clear? why are they significant or meaningful? (2) eval with only one expert could be highly biased and could invite a lot of questions. Or, perhaps you could put this section as "Case Study" as the last section in exp, which is usually just showcasing several examples, and if we choose to framew it as a case study, you only need to compare Claude and ChemAgent(Claude) }

% To evaluate the models' performance in real-world scenarios, we assess them on four expert-proposed tasks selected from the ChemCrow paper \citep{bran2023chemcrow}. 
% We first consulted\hs{engaging domain experts is significant efforts. the word `consult' undersells the contribution.} a domain expert to select tasks that they deem interesting and practical, who eventually selected 4 tasks namely Task 3, 7, 8, and 12 \hs{give a description of what they are and list them in appendix}. These tasks do not have gold standard results, and are designed to evaluate models' comprehensive abilities.
% Subsequently, the models are employed to conduct these tasks and provide detailed final answers. These answers are then evaluated by the domain expert, with model names masked and order randomized to ensure unbiased assessment. Specifically, the domain expert evaluates each answer on whether it adequately addresses the task (1 if task addressed, 0 if not)\hs{what is the difference between `addressed' and `correctness'}, its correctness (1 for fully correct, 0.5 for minor mistakes, 0 for incorrect), and its advantages and disadvantages \hs{compared with what??} in terms of solving the task. Finally, each answer is assigned an overall score from 0 to 10 based on the relative quality of the answers.

% Due to resource constraints and the impracticality of human evaluation for multiple concurrent responses, we limit our evaluation to four models: the base LLM Claude-3.5-Sonnet, ChemCrow (GPT-4), ChemCrow (Claude-3.5-Sonnet), and our \modelname (Claude-3.5-Sonnet). We include the GPT-4-based ChemCrow to compare its performance with the Claude-based version, as the original ChemCrow paper \citep{bran2023chemcrow} uses GPT-4 as its backbone.

% \input{table/cctask}

% The full results are presented in \cref{app:cctask_detail}, with the average scores over the four tasks provided in \cref{tab:cctask}.
% % The results of this analysis show that \modelname's responses are preferred (i.e., achieving the highest score among other models) by our chemistry expert in all but Task 8. In that case, Claude-3.5-Sonnet response scores only slightly higher due to it indicating that the precursors were commercially available while our \modelname does not.
% Our analysis indicates that our proposed model's responses were preferred (i.e., achieved the highest score among other models) by the chemistry expert in all tasks except Task 8. In that instance, Claude-3.5-Sonnet's response scored marginally higher due to its indication of commercially available precursors, which our model did not specify.

% % Notably, the responses from all three agents can always address the tasks. In contrast, Claude-3.5-sonnet without tools refused to answer Task 12, because it does not have the ability to obtain updated material costs as required in the task. This showcases the scenarios where tools for updated information are necessary for certain tasks.
% Overall, all the three agents outperform the base LLM, suggesting the importance and benefit of tools on \cctask.
% Notably, the responses from all three agent-based models consistently addressed the tasks. In contrast, Claude-3.5-Sonnet without tools declined to answer Task 12, citing an inability to obtain updated material costs as required. This underscores scenarios where tools for accessing current information are essential for certain tasks.

% % Interestingly, the disadvantages noted by our expert for each task were similar between ChemAgent and ChemCrow (Claude-3.5-sonnet).
% % For instance, both agents misinterpret methylperoxide to be dimethylperoxide in Task 3.  
% % In Task 4 and 8, both agents struggle with ensuring a full synthesis route to purchasable materials is provided, although ChemAgent does at least provide a route in both cases.
% % This illustrates the importance of the backend model's capabilities for reasoning in the chemistry domain.
% Interestingly, the disadvantages noted by our domain expert for each task were similar between \modelname and ChemCrow (Claude-3.5-Sonnet). For instance, both agents misinterpreted methylperoxide as dimethylperoxide in Task 3. In Tasks 4 and 8, both agents struggled to provide a complete synthesis route to purchasable materials, although our model did offer a partial route in both cases. These observations highlight the importance of the underlying model's reasoning capabilities in the chemistry domain.

% % Additionally, we also observe that ChemCrow (GPT-4) failed to report safety considerations in cctask-8 and cctask-12, while ChemAgent and ChemCrow (Claude-3.5-Sonnet) both address safety concerns in these cases.
% % This pattern suggests that agents based on Claude-3.5-sonnet may have better intuition about material safety.
% % Frazier: I'm not sure if we can really conclude this here based on such a small sample size, but I'm looking for meaning in the analysis we performed.
% Additionally, we observed that ChemCrow (GPT-4) failed to report safety considerations in Tasks 8 and 12, while \modelname and ChemCrow (Claude-3.5-Sonnet) both addressed safety concerns in these instances. This pattern might indicate that agents based on Claude-3.5-Sonnet may possess better intuition regarding material safety.

% % In some cases, all of the responses shared similar disadvantages, regardless of backend model.
% % For example, in Task 3, all of the agents failed to identify the key reason behind the reaction mechanisms.
% % This suggests that both of the backend models lack some necessary chemistry knowledge to effectively use the tools provided and interpret their output.
% % As models continue to improve, we hope to see LLMs that can internalize the nuanced chemistry knowledge necessary for these tasks.
% % Frazier: This needs reworded, and possibly may be more of a discussion point when paired with information about the MMLU analysis.
% In some cases, all responses shared similar disadvantages, regardless of the backend model. For example, in Task 3, all agents failed to identify the key reason behind the reaction mechanisms. This suggests that both backbone models lack some necessary chemistry knowledge to effectively utilize the provided tools and interpret their output. As models continue to evolve, we anticipate the development of LLMs capable of internalizing the nuanced chemistry knowledge required for these tasks.

==> discussion.tex <==
\section{Discussion}
\label{sec:discuss}

% What to discuss?

% Main Takeaways:
% - For specified tasks, agent is better. for more reasining, maybe raw LLMs is better.
% - Different backbone models have different tool calling preference.
% - Tool implementation is important.
% - Information mismatch. How to solve? 

% \textbf{Tooling or not tooling for chemistry problem-solving?}

% Based on our experiments, we can conclude that whether tooling depends on the tasks and the tool sets. 
% On applied chemistry tasks which mainly focus on molecular manipulations, predictions, and representations, at which the current SoTA LLMs are still not good, and there are specific tools for those tasks. In this case, augmenting tools can be very helpful, as the tools can provide accurate information and reliable support for the specialized operations. Also, if the tasks require updated information, it is essential to integrate the necessary tools to let LLMs can at least do them. 
% However, on theoretical chemistry questions, where knowledge and reasoning are more prevail, and LLMs need to use more of their internal knowledge and reasoning to complete the tasks, augmenting tools may hinder the reasoning of the LLMs, let it be prone to more mistakes in the problem solving process, and eventually lead to worse performance.
% Although we draw the conclusions from chemistry problem evaluation, we believe this should apply to broader domains like other scientific disciplines and ...

% Our experimental findings indicate that the effectiveness of tool augmentation in chemical problem-solving is contingent upon both the nature of the task.
% In applied chemistry tasks, which primarily involve molecular manipulations, predictions, and representations, current state-of-the-art Large Language Models (LLMs) exhibit limitations. For these specialized operations, augmenting LLMs with domain-specific tools can significantly enhance performance by providing accurate information and reliable support. Furthermore, in scenarios requiring up-to-date information, the integration of appropriate tools becomes essential to enable LLMs to perform these tasks effectively.
% Conversely, in theoretical chemistry questions that predominantly rely on knowledge retrieval and reasoning, the augmentation of tools may potentially impede the LLMs' cognitive processes. In such cases, LLMs need to leverage their internal knowledge base and reasoning capabilities to a greater extent. The introduction of external tools may disrupt this process, potentially leading to increased errors in problem-solving and ultimately resulting in diminished performance.
% While these conclusions are derived from evaluations in the chemistry domain, we posit that these findings may have broader implications across various scientific disciplines and related fields.

% \textbf{What may be the reasons why tool-augmented LLMs cannot outperform raw LLMs on theoretical chemistry questions? Any potential solutions?}
\textbf{Potential Causes for ChemAgent's Underperformance}

% Based on our observations, we hypothesize there are the following several aspects of reasons:
Based on our observations, we hypothesize several factors:

% (1) LLMs work in a different way in an agent from the way they are pretrained for. Current LLMs are trained with massive human language corpus, so they are more familiar with the content existing in the human world. Since there must be many chemistry questions and solutions in the pretraining data, it's easy for them to recall the related information and respond in a natural logic just as human do. However, when they serve as the backbone in a tool-augmented agent, they are usually provided tools that they may have hardly seen in the training data, and prompted to output in a strange format (e.g., subsequently outputting the thought, and action with certain prefixes, etc). The context for them then becomes a semantic shift, influencing its performance. \citet{shi2023large} also suggests that LLMs can be easily distracted by irrelevant content (the tool-related context and tool output, and the output format, etc., can be some how irrelevant content) and thus reduce the accuracy of its reasoning and output.
LLMs operate differently within an agent framework compared to their pretraining paradigm. During pretraining, LLMs are exposed to vast corpora of human language, including numerous chemistry questions and solutions. This enables them to recall relevant information and respond with human-like logic. However, when integrated into a tool-augmented agent, LLMs encounter unfamiliar tools and are often prompted to generate output in unconventional formats (e.g., structured thought processes and actions with specific prefixes). This semantic shift in context can adversely affect performance. Shi et al. (2023) suggest that LLMs can be easily distracted by irrelevant content, potentially including tool-related context, tool output, and prescribed output formats, which may compromise reasoning accuracy and output quality.

% To this problem, one potential solution is to design new agent framework so that it avoids formatted output at the biggest extent, or employ a multi-agent frameworks to reduce the impact for each LLM instance. Additionally, training of tuning new LLMs with the agent workflow data would help agent get familiar with the workflow, and reduce its impact on reasoning.
Potential solutions include:
a) Designing novel agent frameworks that minimize formatted output requirements.
b) Implementing multi-agent architectures to distribute the impact across multiple LLM instances.
c) Training or fine-tuning new LLMs using agent workflow data to enhance familiarity with the operational paradigm and mitigate its impact on reasoning.


% (2) Tools bring more noises and challenges. Although tools can provide useful information in most cases, they also return incorrect/inaccurate information. This brings many noises for LLMs to identify and the big challenges to verify and use the information.

% To alleviate this problem, models' implementation should be refined, to make the tools robust, universally useful. To avoid multi-source information mismatch, on the one hand, we can design a verification module to help verify the tools' output. A mechanism of confidence in each tool would also be beneficial.

While tools can provide valuable information in many instances, they may also return incorrect or inaccurate data. This introduces noise that LLMs must identify and presents significant challenges in verifying and utilizing the information effectively. Potential solutions include:
a) Refining tool implementations to enhance robustness and universal utility.
b) Developing a verification module to assess tool outputs.
c) Implementing a confidence mechanism for each tool to facilitate more informed decision-making.


% \textbf{What are the other main takeaways?}

% \todo{To extract key ones from experimental analysis.}



% These findings contribute to our understanding of the relative strengths and limitations of different AI model architectures in the domain of chemistry. They also highlight the complexity of effectively integrating domain-specific tools with general language models for specialized scientific tasks. Further research is warranted to elucidate the underlying factors contributing to these performance differentials and to explore potential avenues for improving the efficacy of tool-augmented models in theoretical chemistry applications.



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tool_analysis.tex <==
\subsection{Tool Use Analysis}
\label{sec:exp_tool}

To take a closer look at how \modelname calls tools to solve the input tasks and to understand more about the reasons of the performance disparity between applied chemistry tasks and theoretical chemistry questions, we select \smolinstruct and \mmluc as the representative from each of their categories, and conduct a tool use analysis on them respectively.

\subsubsection{\smolinstruct}

\label{sec:sm_tool}

To investigate the tool use patterns of ChemAgent, we classify the tool chain (i.e., the sequence of the used tools) into three types:

\begin{itemize}[leftmargin=*]
    \item \textbf{Direct}: Directly using the related tool(s) in the most straightforward way to solve the problems, without calling any other tools. For example, on the forward synthesis task, the direct tool chain is ``ForwardSynthesis $\rightarrow$ Answer''; on the name conversion task, IUPAC to Formula, the direct tool chain is ``IUPAC2SMILES $\rightarrow$ SMILES2Formula.''\footnote{The direct tool chains are manually defined based on task definitions and the available tool set, which can be found in \cref{app:direct_tool_chain_sm}}
    \item \textbf{Supportive}: Calling other tools besides for the tools in the direct tool chain. This usually happens when agent tries to convert the input to a certain format, or using other information sources to verify its answer, although some are not necessary.
    \item \textbf{Unconventional}: Using all\hs{all? do you mean all tools used in this type of tool chains never appear? } the other tools that never appear in the direct tool chain. \hs{the naming, `supportive' and `unconventional', is confusing and inappropriate. might call them, `direct' - 'redundant' - `missing'}
\end{itemize}


\input{figure/chemagent_smolinstruct_tool_statistics}

The statistics result for each task is presented in \cref{fig:chemagent_sm_tool}. We can have the following observations:

(1) ChemAgent demonstrates a strong tendency towards direct tool chain utilization across all tasks, with a significant proportion of interactions falling into the Direct and Supportive category, particularly in the Claude-based model. Despite being provided with an extensive toolkit of over 20 tools, many of which are not directly applicable to the given tasks, and only textual descriptions without examples, for the tasks in SMoIInstruct, both ChemAgent models demonstrate a clear understanding of the objectives and exhibit a remarkable ability to discern and select appropriate tools without being distracted by extraneous options.

(2) In a small percentage of cases, particularly evident in the Claude-based model, the agents employ tools outside the direct tool chain, which, However, is often still logically sound according to our observation. For instance, in the Molecule Generation task, where ChemAgent is tasked with generating or designing a molecule based on a textual description, some instances show the model opting for the PubchemSearchQA tool instead of the more direct MoleculeGenerator. This approach involves obtaining information about a related molecule mentioned in the description, modifying it as needed, and then re-verifying the designed molecule's compliance with the given requirements using PubchemSearchQA. This adaptive strategy further underscores the LLMs' comprehension of task requirements and their ability to leverage tools in a reasoned and flexible manner.

(3) A distinct difference in tool use patterns emerges when comparing the GPT and Claude backbones. The GPT-based ChemAgent exhibits a stronger preference for direct tool use, with 94\% of interactions falling into this category, indicating a more streamlined and efficient approach. In contrast, the Claude-based ChemAgent shows a more balanced distribution, with 63\% direct use and a significant 35\% supportive use. This suggests that the Claude model tends to adopt a more exploratory and potentially thorough approach, often employing additional tools for result verification or supplementary information gathering. While this strategy may lead to more robust and verified results in some scenarios, it is important to note that when faced with inconsistent information from multiple sources, it could potentially lead to confusion and erroneous outputs.
See a case in \cref{app:} for more details.
% The implications of these differing approaches warrant further investigation in subsequent sections, particularly through detailed case studies.


\subsubsection{\mmluc}
\label{sec:mmluc_tool}


